Spatial Fluid Limits for Stochastic Mobile Networks

We consider Markov models of large-scale networks where nodes are characterized by their local behavior and by a mobility model over a two-dimensional lattice. By assuming random walk, we prove convergence to a system of partial differential equations (PDEs) whose size depends neither on the lattice size nor on the population of nodes. This provides a macroscopic view of the model which approximates discrete stochastic movements with continuous deterministic diffusions. We illustrate the practical applicability of this result by modeling a network of mobile nodes with on/off behavior performing file transfers with connectivity to 802.11 access points. By means of an empirical validation against discrete-event simulation we show high quality of the PDE approximation even for low populations and coarse lattices. In addition, we confirm the computational advantage in using the PDE limit over a traditional ordinary differential equation limit where the lattice is modeled discretely, yielding speed-ups of up to two orders of magnitude.

==> validation.tex <==
% !TEX root = ssf.tex


\section{Validation}\label{sec:validation}

The goal of this section is to provide evidence on the convergence of the PDE solution. In Section~\ref{sec:validation-si} we consider the simple spatial model of epidemics introduced in Section~\ref{sec_general} to illustrate our general framework. In this case, the locally Lipschitz continuity of the reactive terms yield convergence for DBCs. Here, we present results that numerically demonstrate the quality of such convergence as a function of the lattice size $K$. In Section~\ref{sec:validation-min} we consider a different example, with 6 local states, exhibiting globally Lipschitz reactive terms based on minimum functions in order to model capacity sharing mechanisms. We use DBCs to further demonstrate convergence  numerically. In addition, we also consider NBCs. Although  convergence cannot be established formally in this case, we show that, under the experimental conditions set for our study, the PDE solution is nevertheless a very accurate estimate of the stochastic process, analyzed by means of very costly simulation, for increasing values of $K$ and $N$.

Throughout this section, we will make use of the following function in order to set-up the initial conditions for our models, consistently with both DBCs and NBCs:
\[
\theta(x,y)\! = \!\begin{cases}
0 \!\!\! &,  \ \lVert (x,y) - (\frac{1}{2},\frac{1}{2}) \rVert ^2 \geq \frac{1}{4} \\
\frac{\text{exp}(4)}{\text{exp}\left( 1 /(\frac{1}{4} - \lVert (x,y) - (\frac{1}{2},\frac{1}{2}) \rVert ^2 )\right)} \!\!\! &, \
\text{otherwise.}
\end{cases}
\]
It has a global maximum at $(\frac{1}{2},\frac{1}{2})$ and vanishes towards the boundary of $[0;1]$.

\subsection{Epidemics Model}\label{sec:validation-si}

\begin{figure}
\includegraphics[scale=0.6]{si0-eps-converted-to}\hfill
\includegraphics[scale=0.6]{si5-eps-converted-to}\hfill
\includegraphics[scale=0.6]{si10-eps-converted-to}
\caption{Initial condition (left plot) and solution at times $t= 5.0$  and $t=10.0$ (middle and right plots, respectively) for $\alpha_1(x,y)$ solution to the epidemics model of Section~\ref{sec:validation-si}.}\label{fig:si}
\end{figure}

\paragraph*{Parametrization} We use DBCs and fix as initial populations and parameters
\begin{equation}\label{eq:si.dbc}
\alpha_1^0(x,y) = 0.2 \cdot \theta(x,y), \qquad \alpha_2^0(x,y) = 0.5 \cdot \theta(x,y), \qquad \beta_1^1(x,y) = 1.0 \qquad \text{and} \qquad  \beta^2_1(x,y) = 0.7 \cdot \theta(x,y) .
\end{equation}
In particular, we assume that exogenous arrivals are more concentrated in the center of the spatial domain and become 0 at the borders. We arbitrarily fix $t = 10.0$ as the time of interest for our analysis. With this choice of parameters, the PDE solution shows a different configuration than the initial conditions, which is however nontrivially zero due to the fact that not all agent densities have been absorbed by the boundary. To confirm this, Figure~\ref{fig:si} shows the concentrations of susceptibles given by the initial conditions and at time points $t=5.0$ and $t=10.0$. These were obtained with a solver for the Euler finite difference scheme implemented in Matlab, setting $K=16$ and $\Delta = 0.003$; the latter is the time step of choice throughout the remainder of this section.

On a side note, it is interesting to observe an intrinsically competitive behavior between the arrival rate, which initially tends to increase the density of the susceptible individuals, and the impact of the infection and of the boundary absorption, which tends to decrease it in the long term, for this parametrization.

\paragraph*{Convergence of the PDE scheme}
\begin{table}[t]
\centering
\begin{tabular}{rccr}
\toprule
$K$ & $\alpha_1$ & $\alpha_2$ & \emph{Runtime} \\
\midrule
8 &  0.0901 & 0.0416 & 0.75\,s \\
16 & 0.1017 & 0.4329 & 2.86\,s \\
 32 & 0.1081 & 0.4364 & 12.04\,s\\
  64 &  0.1114 & 0.4368 &  49.82\,s\\
   82 & 0.1122 & 0.4368 & 84.79\,s\\
   98 &  0.1126 & 0.4368 & 114.78\,s\\
\bottomrule
\end{tabular}
\caption{Numerical convergence for the PDE finite difference scheme with DBCs (\ref{eq:si.dbc}) for the epidemics model. Average densities $\alpha_1(x,y)$ and $\alpha_2(x,y)$ across all regions at time $t = 10.0$.}\label{tab:si}
\end{table}

Table~\ref{tab:si} shows the results of the PDE scheme as a function of $K$. As a representative performance index, we take the average densities of susceptibles and individuals across all regions at time $t=10.0$. For each $K$, we display the average runtimes measured on commodity hardware over 30 independent samples. Convergence is numerically demonstrated by the fact that for larger $K$ the relative distance between solutions becomes smaller---for instance the average density for $\alpha_2$ stabilizes up to the fourth decimal digit for $K \geq 64$. As expected, however, $K$ has a dramatic impact on the computation time.

\subsection{Capacity Sharing Model}\label{sec:validation-min}
\paragraph*{Model description} We now turn to a spatial model with local interactions of resource-sharing type. Here we consider an example with $L=6$ agent types and  the following rate functions:
%,
\begin{align*}
F_1(A_1, \ldots, A_6) & =  \min (A_1,A_3), & \!\! c_{11} \! = c_{13} \! = d_{12}\!  = d_{14}  & = \!1, \\
F_2(A_1, \ldots, A_6) & = \min (A_2,A_5),& \!\! c_{22} \! = c_{25} \! = d_{11} \! = d_{26}  & = \!1,  \\
F_3(A_1, \ldots, A_6) & =  \min (A_4,A_6), & \!\! c_{43} \! = c_{36} \! = d_{33} \! = d_{35}  & = \!1,
\end{align*}
with all other $c_{jl}$ and $d_{j'l'}$ being equal to $0$,  for $1 \leq j,j' \leq 3$ and $1\leq l,l' \leq 6$.
Intuitively, this model could represent, in each region, a queueing network with three multi-server stations where both clients and servers change state upon service. For instance, if $A_1$ has the interpretation of a client population and $A_3$ is a server population, by the first reaction we have that $A_1$ changes state to $A_2$ and $A_3$ becomes $A_4$. Let us recall that local interactions take place between agents within the same domain.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph*{Parametrization} We fix $\mu_1 =  \mu_2 = \mu_3 = 0.01$. We also experimented with other values but the results are qualitatively similar to those considered here, thus they are omitted for space reasons. The initial conditions are chosen as follows.

As discussed, for this model we consider both NBCs and DBCs. In particular, we study two distinct NBC configurations because, as will be numerically shown later, this model may feature different regimes of quasi equilibrium depending on the initial configurations. Thus, we study whether this fact has a significant influence on the quality of the numerical convergence.

The first NBC configuration is:
\begin{align}
\alpha_1^0(x,y) & = \frac{2}{5}, & \!\!\!\alpha_2^0(x,y) & = 0, & \!\!\!\alpha_3^0(x,y) & = \frac{2}{5}, \notag \\
\alpha_4^0(x,y) & = 0, & \!\!\!\alpha_5^0(x,y)  & = \theta(x,y), &  \!\!\!\alpha_6^0(x,y)  & = 0 . \label{eq:first.ic}
\end{align}

The second NBC configuration is:
\begin{align}
\alpha_1^0(x,y) & = \frac{2}{5},   & \!\!\!\alpha_2^0(x,y) & = 0, & \!\!\!\alpha_3^0(x,y) & = \frac{2}{5}, \label{eq:second.ic} \\
\alpha_4^0(x,y) & = 0, & \!\!\!\alpha_5^0(x,y)  & = \frac{1}{2}\theta(x,y), &  \!\!\!\alpha_6^0(x,y)  & = \frac{1}{2}\theta(x,y). \notag
\end{align}


\begin{figure}
\includegraphics[scale=0.9]{cs_t0-eps-converted-to}\hfill
\includegraphics[scale=0.9]{cs_t30-eps-converted-to}
\caption{Initial condition (left plot) and solution at time $t= 30.0$ (right) for $\alpha_5(x,y)$ with NBCs  (\ref{eq:first.ic}).}\label{fig:cs-stat}
\end{figure}
With both parameterizations, we found that $t = 30.0$ gives a good approximation to a stationary regime for both initial configurations, as at further time steps the solutions does not change with precision up to the fourth decimal digit. For illustration, Figure~\ref{fig:cs-stat} shows the initial configuration (\ref{eq:first.ic}) and the PDE solution at $t=30.0$ for $\alpha_5(x,y)$ by setting $K = 16$.

\begin{figure}
\includegraphics[scale=0.9]{dirichlet1-eps-converted-to}\hfill
\includegraphics[scale=0.9]{dirichlet5-eps-converted-to}
\caption{Solutions at times $t = 1.0$ (left) and  $t= 5.0$ (right)  for $\alpha_5(x,y)$ with DBC (\ref{eq:dirichlet}). The initial condition corresponds to the left plot of Figure~\ref{fig:cs-stat}.}\label{fig:dirichlet}
\end{figure}
For DBCs, we take the configuration
\begin{align}
\alpha_1^0(x,y) & = \frac{\theta(x,y)}{5}, & \!\!\!\alpha_2^0(x,y) & = 0, & \!\!\!\alpha_3^0(x,y) & = \frac{\theta(x,y)}{10}, \notag \\
\alpha_4^0(x,y) & = 0, & \!\!\!\alpha_5^0(x,y)  & = \theta(x,y), &  \!\!\!\alpha_6^0(x,y)  & = 0. \label{eq:dirichlet}
\end{align}
We consider the transient PDE solution, as in our study concentrations tend to exit the spatial domain in the long term. In this case, we considered $t = 5.0$ as a time point of interest, since the solution is sufficiently away from the initial conditions yet not close to 0. With this choice of parameters, the predicted fraction of the density of agents of  type $A_5$ still within the boundary is ca 48\%. Figure~\ref{fig:dirichlet} illustrates the tendency to extinction of $\alpha_5$ by plotting the solution at times $1.0$ and $5.0$; the functions $\alpha_2^0(x,y)$ and $\alpha_5^0(x,y)$ are equal for all boundary conditions considered here, and thus they can be seen in the left plot of Figure~\ref{fig:cs-stat}.

\begin{table}[t]
\centering
\begin{tabular}{rccccr}
\toprule
& \multicolumn{2}{c}{$\alpha_2$} & \multicolumn{2}{c}{$\alpha_5$} \\
\cmidrule(l){2-3}  \cmidrule(l){4-5}
\multicolumn{1}{c}{$K$} &  \emph{Eq. \ref{eq:first.ic}}  & \emph{Eq. \ref{eq:second.ic}} & \emph{Eq. \ref{eq:first.ic}}  & \emph{Eq. \ref{eq:second.ic}}  & \multicolumn{1}{c}{\emph{Runtime}} \\
\midrule
8 &   0.2916 & 0.3458 &  0.0542 & 0.0542&1.96\,s \\
16 &     0.2785 & 0.3393 &   0.0607 &0.0607 &6.59\,s \\
 32 &   0.2710   & 0.3355 &0.0645 &0.0645 & 24.67\,s \\
  64 &  0.2670   & 0.3335  &0.0665 & 0.0665 &100.11\,s \\
   82 & 0.2661   & 0.3331 & 0.0669 &0.0669 &163.55\,s \\
   98 &  0.2657  & 0.3328  &0.0672 &0.0672 &231.07\,s\\
\bottomrule
\end{tabular}
\caption{Numerical convergence for the PDE finite difference scheme with NBCs. Average densities $\alpha_2(x,y)$ and $\alpha_5(x,y)$ across all regions at time $t = 30.0$.}\label{tab:convergence.nbc}
\end{table}

\begin{table}[t]
\centering
\begin{tabular}{rccr}
\toprule
$K$ & $\alpha_2$ & $\alpha_5$ & \emph{Runtime} \\
\midrule
8 &  0.0018 & 0.0522 & 1.37\,s \\
16 & 0.0020 & 0.0592 & 4.98\,s \\
 32 &0.0022 & 0.0630 & 19.94\,s\\
  64 &  0.0022 & 0.0650 & 82.50\,s\\
   82 & 0.0023  & 0.0655 & 136.66\,s\\
   98 &  0.0023  & 0.0657 & 188.65\,s\\
\bottomrule
\end{tabular}
\caption{Numerical convergence for the PDE finite difference scheme with DBCs (\ref{eq:dirichlet}). Average densities $\alpha_2(x,y)$ and $\alpha_5(x,y)$ across all regions at time $t = 5.0$.}\label{tab:convergence.dbc}
\end{table}

\paragraph*{Convergence of the PDE scheme}
For the NBCs conditions, the results of Section~\ref{sec_general} guarantee that the scheme is stable, that is, the error remains bounded as $\dt, 1/K \rightarrow 0$. Table~\ref{tab:convergence.nbc} shows the estimates of the average population densities $\alpha_2(x,y)$ and $\alpha_5(x,y)$ at time $t = 30.0$ across all regions for both NBC conditions (\ref{eq:first.ic}) and (\ref{eq:second.ic}). Similarly to the results in Table~\ref{tab:si}, all estimates tend to convergence with increasing $K$. The table also numerically confirms the existence of the two quasi-equilibria regimes, although $\alpha_2(x,y)$ is insensitive up to the fourth decimal digit.  Compared to the runtimes of Table~\ref{tab:si}, this model has longer runtimes for each $K$: clearly this is due to the larger number of local states $L$.

Table~\ref{tab:convergence.dbc} reports the same results for the DBCs (\ref{eq:dirichlet}), for which convergence of the PDE finite difference scheme is ensured by Theorems \ref{thm_scheme} and \ref{thm_main}. It can be seen that the behavior of the solution as a function of $K$ follows a similar trend to Table~\ref{tab:convergence.nbc}.

Overall, these observations seem to suggest the fact that, although only stability can be proved  theoretically for NBCs, in practice the scheme seems to converge. Unfortunately, it is not possible to check this precisely because an analytical solution for our model under consideration is not available.  However, in order to gain more confidence on the use of the finite difference scheme also for NBCs, in the following we compare the PDE estimates against the \emph{true} behavior of the system intended as the dynamics of the stochastic process.


\paragraph*{Convergence of the stochastic process} We perform this evaluation  by considering different CTMCs with initial conditions determined by Eq.~\ref{eq:first.ic} (using the NBCs of Eq.~\ref{eq:second.ic} does not lead to quantitatively different insights) where $K$ and $N$ are varied whilst all other parameters are kept fixed. Even for small $K$ and $N$ the state space becomes infeasible to enumerate explicitly, therefore we resort to simulation for the evaluation. For each model we perform $500$ independent replicas. As a representative index, we consider the average number of agents in state $A_5$ across all regions at time $t = 30.0$. We take this index as the \emph{exact} value  that we wish to approximate and we compare it with the PDE solution, obtained as described above. We define the \emph{approximation error} as the absolute percentage relative error with respect to the average obtained by simulation.

We also give an indication of the cost of the simulation, expressed as the overall wall-clock execution time to sample all the independent 500 realizations. In practice, however, each realization was computed on an independent core in a cluster environment (using a simulator implemented in Java). Due to the excessively large computational effort required, runtime measurements were only taken once.


\begin{table}[t]
\centering
\begin{tabular}{rrcccc}
\toprule
&&\multicolumn{2}{c}{\emph{Simulation}} & \multicolumn{2}{c}{\emph{PDE}} \\
\cmidrule(l){3-4} \cmidrule(l){5-6}
\multicolumn{1}{c}{$N$} & \multicolumn{1}{c}{$K$} & \emph{\# $A_5$} & \emph{Runtime} &  \emph{\# $A_5$} & \emph{Error}   \\
&&& \emph{\scriptsize{DD:HH:MM}} \\%&&  & & \emph{\scriptsize{($ds = 1/64$,}}\\
%&&&&& \emph{\scriptsize$\alpha = 0.066$)} \\
\midrule
 $25$ & $8$ & $1.315 \pm 0.12$ & 00:03:15 & $1.355$ & $3.04\%$ \\
 $50$ & $8$ & $2.651 \pm 0.16$ & 00:06:28 & $2.710$ & $2.23\%$ \\
$100$ & $8$ & $5.331 \pm 0.22$ & 00:12:47 &$5.420$ & $1.67\%$ \\
\midrule
$25$ & $16$ & $1.409 \pm 0.12$ & 04:17:06 & $1.517$ & $7.70\%$\\
 $50$ & $16$  & $2.922 \pm 0.16$ & 09:11:07 & $3.035$ & $3.87\%$ \\
 $100$ & $16$ & $5.967 \pm 0.23$ & 18:23:26 & $6.070$& $1.69\%$ \\
\midrule
$25$ & $32$ & $1.508 \pm 0.08$ & > 6 months &  $1.612$ & $6.92\%$ \\
 $50$ & $32$& $3.104 \pm 0.12$ & > 1 year~ & $3.225$ & $3.90\%$ \\
$100$ & $32$ & $6.340 \pm 0.22$ & > 3 years & $6.450$ & $1.70\%$ \\
\bottomrule
 \end{tabular}
 \caption{Estimates of the total population of $A_5$ at time $t = 30.0$ for varying $N$ and $K$, with NBCs as in (\ref{eq:first.ic}). Simulation averages are computed over 500 realizations and are shown with the maximum 95\% confidence interval across all regions.}\label{tab:capacity}
\end{table}
%
%
The results are shown in Table~\ref{tab:capacity}. The density of $A_5$-agents, as evaluated by simulation, increases with $K$ and follows the trend predicted by the PDE solution shown in Table~\ref{tab:convergence.nbc}. Furthermore, the larger $N$ the higher the quality of the approximation. The approximation results obtained for $N = 100$ allow us to conclude that our finite difference scheme may provide excellent approximations also for solutions to NBCs.

\subsection{Discussion} The numerical evidence provided in this section has shown that the complexity of Markov population processes with explicit locality models defy current computational capabilities, as the cost of analysis grows quickly with $N$ and $K$. In contrast, our PDE interpretation is independent from $N$, as per standard fluid limit, and that it scales well with  $K$, by exploiting the fact that deterministic estimates for large $K$ may be obtained using coarser meshes. We wish to make two noteworthy observations for the practical applicability of these results. First, PDE estimates lead to very small approximation errors for large $N$, which makes this technique particularly appropriate for the analysis of large-scale systems. The second observation is that the PDE solution can be up to seven orders of magnitude faster than simulation, which makes this approach relevant, for instance, in the case where many variants are to be considered, e.g., for capacity planning purposes.



